Stable Matchings with Restricted Preferences: Structure and Complexity

It is well known that every stable matching instance $I$ has a rotation poset $R(I)$ that can be computed efficiently and the downsets of $R(I)$ are in one-to-one correspondence with the stable matchings of $I$. Furthermore, for every poset $P$, an instance $I(P)$ can be constructed efficiently so that the rotation poset of $I(P)$ is isomorphic to $P$. In this case, we say that $I(P)$ realizes $P$. Many researchers exploit the rotation poset of an instance to develop fast algorithms or to establish the hardness of stable matching problems. In order to gain a parameterized understanding of the complexity of sampling stable matchings, Bhatnagar et al. [SODA 2008] introduced stable matching instances whose preference lists are restricted but nevertheless model situations that arise in practice. In this paper, we study four such parameterized restrictions; our goal is to characterize the rotation posets that arise from these models: $k$-bounded, $k$-attribute, $(k_1, k_2)$-list, $k$-range. We prove that there is a constant $k$ so that every rotation poset is realized by some instance in the first three models for some fixed constant $k$. We describe efficient algorithms for constructing such instances given the Hasse diagram of a poset. As a consequence, the fundamental problem of counting stable matchings remains $\#$BIS-complete even for these restricted instances. For $k$-range preferences, we show that a poset $P$ is realizable if and only if the Hasse diagram of $P$ has pathwidth bounded by functions of $k$. Using this characterization, we show that the following problems are fixed parameter tractable when parametrized by the range of the instance: exactly counting and uniformly sampling stable matchings, finding median, sex-equal, and balanced stable matchings.

==> downsets.tex <==
\section{FPT Algorithms for Counting and Sampling Downsets}

In this section, we describe FPT algorithms for counting and sampling downsets in DAGs parametrized by (undirected) pathwidth. Throughout the section, we assume that $G = (V, E)$ is a DAG with $p = \abs{V}$ vertices. Given $u, v \in V$, we say $u$ is an \dft{ancestor} of $v$ and $v$ is a \dft{descendant} of $u$ if there is a directed path from $u$ to $v$ in $G$.  We say that $Z \subseteq V$ is a \dft{downset} of $G$ if, for every vertex $v \in Z$, all the ancestors of $v$ also belong to $Z$.

Observe that if $Z$ is a downset in $G$, then $Z$ is a downset in the transitive closure of $G$, and vice versa. Thus, counting and sampling downsets in DAGs are equivalent to counting downsets in posets: in order to count or sample downsets in a poset $\calP$, it suffices to count or sample downsets in any transitive reduction of $\calP$.

Finally, we assume that a simple path decomposition $\calX$ of a DAG $G$ is provided as input to our algorithms. By Theorem~\ref{thm:pathwidth}, there is an FPT algorithm for finding $\calX$ from $G$, so taking $\calX$ as additional input is essentially without loss of generality.

\subsection{Counting Downsets in Pathwidth Bounded DAGs}
\label{sec:counting-downsets}

%% In this section, we will show there is an FPT algorithm for counting all the downsets of a poset $\calP$, by translating the problem in the context of directed acyclic graphs (DAGs).

%% Let $G=(V,E)$ be a DAG with $n$ vertices.
 
Assume that $\pw(G) = k$. Let $\calX = (X_1, X_2, \ldots X_{2n})$ be a simple path decomposition of $G$ with width $k$. For completeness, set $X_0 = \varnothing$. We say that $v$ is \dft{inserted at step $i$} if $X_{i} = X_{i - 1} \cup \set{v}$, and that $v$ is \dft{removed at step $i$} if $X_{i} = X_{i-1} \setminus \set{v}$.  Define the sets $V_1, V_2, \ldots, V_{2n} (= V)$ as
\begin{equation*}
  V_i = \bigcup_{j \leq i} X_j.
\end{equation*}
Finally, let $G_i = G|_{V_i}$, the subgraph of $G$ induced by $V_i$.

The algorithm we present computes the number of closed subsets of $G_i$ for each $i \in [2n]$.  More specifically, it recursively computes $C_i(A)$ for each $i \in [2n]$ and $A \subseteq X_i$ such that
\[
C_i(A) = \abs{\set{Z \subseteq V_i \sucht Z \text{ is a closed subset of } G_i \text{ and } Z \cap X_i = A}}.
\]
Thus, the number of closed subsets of $G_i$ is equal to $\sum_{A \subseteq X_i} C_i(A)$, and the number of closed subsets of $G$ is $C_{2p}(\varnothing) + C_{2p}(X_{2p})$.

Here is the rule that updates $C_{i+1}$  from $C_i$. Let $v_i$ denote the vertex added  or removed  at step $i$. Let $U_i$ and $W_i$ denote $v_i$'s in- and out-neighbors in $G_i$ respectively:
\[
U_i = \set{u \in V_i \sucht (u, v_i) \in E}, \qquad W_i = \set{w \in V_i \sucht (v_i, w) \in E}.
\]
%That is, in $\calP_i$, the elements of $U_i$ are exactly the elements that cover $v_i$  while $v_i$ covers exactly  the elements in $W_i$.  
The update procedure for $C_i$  has two cases, corresponding to $i$ being an insertion event and a removal event.

\begin{description}
\item[Initialize.] $C_0(\varnothing) = 1$.
\item[Insertion.] $v_i$ is inserted at step $i$: for each $A \subseteq X_i$,
  \begin{equation}
    \label{eqn:insert}
  C_i(A) =
  \begin{cases}
    0 &\text{if } A \cap (W_i \cup \set{v_i}) \neq \varnothing, \text{ and } U_i \cup \set{v_i} \nsubseteq A\\
    C_{i-1}(A) &\text{if } A \cap (W_i \cup \set{v_i}) = \varnothing\\
    C_{i-1}(A \setminus \set{v_i})   &\text{ otherwise.}
  \end{cases}
  \end{equation}
\item[Removal.] $v_i$ is removed at step $i$: for each $A \subseteq X_i$,
  \begin{equation}
    \label{eqn:remove}
  C_i(A) = C_{i-1}(A) + C_{i-1}(A \cup \set{v_i})
  %% \begin{cases}
  %%   %0 &\text{if } v_i \in a\\
  %%   C_{i-1}(a) + C_{i-1}(a \cup \set{v_i}) &\text{if } U_i \subseteq a, W_i \cap a = \varnothing\\
  %%   C_{i-1}(a \cup \set{v_i}) &\text{if } W_i \cap a \neq \varnothing\\
  %%   C_{i-1}(a) &\text{otherwise.}
  %% \end{cases}
  \end{equation}
\end{description}

The following lemma asserts the correctness of the formulas described above.

\begin{lem}
  \label{lem:count-update}
  %Let $H_\calP$ be the Hasse diagram of $\calP$ that has $p$ elements,  and let $v_1, v_2, \ldots, v_{2p}$ be the of vertices described above. Then 
  For each $i \in [2n]$ and $A \subseteq X_i$, the recursive formulas in (\ref{eqn:insert}) and (\ref{eqn:remove}) imply  %we have
  \[
  C_i(A) = \abs{\set{Z \subseteq V_i \sucht Z \text{ is a closed subset of } G_i \text{ and } Z \cap X_i = A}}.
  \]
\end{lem}

\begin{proof}
  We argue by induction on $i$. For the base case $i = 1$, the vertex $v_1$ is added to $X_1$, and $V_1 = \set{v_1}$. Thus $\calP_1$ consists of a single element. By the description of the insertion procedure, we have
  \[
  C_1(\varnothing) = 1, \qquad C_1(\set{v_1}) = 1,
  \]
  which are the correct counts.

  For the inductive step, assume the conclusion of the lemma holds for $i - 1$. That is, for all $A \subseteq X_{i-1}$ we have
  \[
  C_{i-1}(A) = \abs{\set{Z \subseteq V_{i-1} \sucht Z \text{ is a closed subset of } \calP_{i-1} \text{ and } Z \cap X_{i-1} = A}}.
  \]
  We consider insertions and removals separately. First, suppose vertex $v_i$ is inserted at step $i$; i.e, $X_i = X_{i-1} \cup \{v_i\}$.   We begin by establishing the fact that $U_i \cup W_i \subseteq X_i$.

  
   Let $(u, v_i)$ be an edge of  $G$ and $u \in V_i$.   If $u \not \in X_i$, then $u$ was inserted and removed at steps earlier than $i$ in $\calX$.  Consequently,  $u$ and $v_i$ will never appear together in some set of $\calX$, violating the fact that $\calX$ is a path decomposition of $G$.  By the same argument,  if $(v_i, w)$ is an edge of $G$ and $w \in V_i$ then $w \in X_i$.   Hence, $U_i \cup W_i \subseteq X_i$.

   
 %  Otherwise, in $\calX$, $u$ is inserted and removed at steps earlier than $i$.    
   %Thus, $U_i \cup W_i \subseteq X_i$.
  
   %Since $\calX$ is a path decomposition, $U_i \cup W_i \subseteq X_i$.  That is, all the elements that cover $v_i$ and all the elements that $v_i$ covers in $\calP_i$ belong to $X_i$.  
   
    Fix a subset $A \subseteq X_i$. We address the three cases  in Equation~(\ref{eqn:insert}):
  \begin{description}
  \item[$A \cap (W_i \cup \set{v_i}) \neq \varnothing, U_i \cup \set{v_i} \nsubseteq A$.] In this case,  $A$ contains $v_i$ or some of $v_i$'s out-neighbors but not  $v_i$ and all of $v_i$'s in-neighbors in $G_i$.  If $Z \cap X_i = A$, then $Z$ cannot be a closed subset of $G_i$. Thus $C_i(A) = 0$.
   
 % there is no downset $Z \subseteq V_i$ with $Z \cap X_i = A$ because some of the predecessors of $A \cap (W_i \cup \set{v_i})$ are missing from $Z$.  Thus, $C_i(A) = 0$.
  %  as there is a directed path (of length $1$ or $2$) from every vertex $u \in U_i$ to every vertex $w \in W_i \cup \set{v_i}$. Thus $C_i(a) = 0$.
  \item[$A \cap (W_i \cup \set{v_i}) = \varnothing$.]  For this case, we claim that $Z$ is a closed subset of $G_i$ with $Z \cap X_i = A$ if and only if $Z$ is a closed subset of $G_{i-1}$ with $Z \cap X_{i-1} = A$. The equality $C_i(A) = C_{i-1}(A)$ follows.

It is easy to see that closed subsets of $G_i$ that do not contain $v_i$  are also closed subsets of $G_{i-1}$.  Thus, if $Z$ is a closed subset of $G_i$ with $Z \cap X_i = A$ and $A \cap \set{v_i} = \varnothing$, then $Z$ is a closed subset of $G_{i-1}$. And since $v_i \not \in Z$, $Z \cap X_{i-1} = A$.  

It is also straightforward to verify that closed subsets of $G_{i-1}$ that do not contain any vertices in $W_i$ are also closed subsets of $G_i$.  Thus, if $Z$ is a closed subset of $G_{i-1}$ with $Z \cap X_{i-1} = A$ and $A \cap W_i  = \varnothing$, then $Z$ is a closed subset of $G_{i}$.  Furthermore, $Z \cap X_i = A$ because $v_i \not \in A$.  



  %  First suppose $Z$ is a downset of $G_i$ with $Z \cap X_i = A$. Since $A$ does not contain $v_i$, we have $Z \subseteq V_{i-1}$. Moreover, $Z$ is a downset of $G_{i-1}$ because every directed path in $G_{i-1}$ is also a directed path in $G_i$.

 %   Now suppose $Z$ is a downset in $G_{i-1}$ with $Z \cap X_{i-1} = A$. Since $Z$ is a downset and does not contain any element $w \in W_i$, $Z$ does not contain any descendant of $w$, nor any descendant of $a$. Thus for every $v \in Z$, all ancestors of $v$ in $G_i$ are also ancestors of $v$ in $G_{i-1}$. Therefore, every ancestor of each $v \in Z$ in $G_i$ is also contained in $Z$, hence $Z$ is a downset in $G_i$.
 
 
  \item[Remaining case.]  If the first and second conditions are not true, then 
  %$A \cap (W_i \cup \set{v_i}) = \varnothing$ or  $U_i \cup \set{v_i} \subseteq A$.  If additionally the second case is not true then 
  $A \cap (W_i \cup \set{v_i}) \neq \varnothing$ and  $U_i \cup \set{v_i} \subseteq A$.  But $U_i \cup \set{v_i} \subseteq A$ implies that $A \cap (W_i \cup \set{v_i}) \neq \varnothing$ because $v_i \in A$.  So we shall just assume that $U_i \cup \set{v_i} \subseteq A$.
  
     We claim that $Z$ is a closed subset of $G_i$ with $Z \cap X_i = A$  if and only if  $Z' = Z \setminus \set{v_i}$ is a closed subset of $G_{i-1}$ with $Z' \cap X_{i-1} = A \setminus \set{v_i}$. The equation $C_{i}(A) = C_{i-1}(A \setminus \set{v_i})$ follows.
  %$Z \setminus \set{v_i}$ is a downset of $\calP_{i-1}$. 
  
  %$A \cap (W_i \cup \set{v_i}) \neq \varnothing$, and $U_i \cup \set{v_i} \subseteq A$.  That is,  $A$ contains $v_i$ and all the elements that cover $v_i$ in $\calP_i$ and none or some of the elements it covers as well as all the elements that cover $
%  Consider downset $Z$ of $\calP_i$.  For an arbitrary $z \in Z$, if $a \neq v_i$ is a predecessor of $z$ in $\calP_i$, then $a$ is still a predecessor of 
  
  %Consider an arbitrary element $x \in V_i$, $x \neq v_i$.  Notice that $a \neq v_i$ is a predecessor of $x$ in $\calP_i$ if and only if  $a$ is a predecessor of $x$ in $\calP_{i-1}$.  On the other hand, if $v_i$ is a predecessor of $x$ in $\calP_i$, it no longer is one in $\calP_{i-1}$ since $v_i \not \in V_{i-1}$.   Thus,  
  
  Notice that  if $Z$ is a closed subset of $G_i$ and $v_i \in Z$, then $Z \setminus \set{v_i}$ is a closed subset of $G_{i-1}$.  And if $Z \cap X_i = A$ then $(Z\setminus \{v_i\}) \cap X_{i-1} = A \setminus \{v_i \}$. 
  
  Next, assume $Z'$ is a closed subset of $G_{i-1}$ such that $U_{i} \subseteq Z' \cap X_{i-1}$.  Then all the in-neighbors of $v_i$ in $G_i$ are in $Z'$ so $Z' \cup \set{v_i}$ is a closed subset of $G_i$.  If $Z' \cap X_{i-1} = A'$ then $(Z' \cup \set{v_i}) \cap X_i = A' \cup \{v_i \}$.
  

 %   First suppose $Z$ is a downset in $\calP_i$. As before, every path in $G_{i-1}$ is a path in $G_i$. Since for each $z \in Z \setminus \set{v_i}$, every ancestor of $z \in G_i$ is in $Z$, every ancestor of $z$ in $G_{i-1}$ is also in $Z$. Thus $Z$ is closed in $G_{i_1}$.

  %  Now suppose $Z \setminus \set{v_i}$ is a downset in $G_{i-1}$, and let $z \in Z$. Suppose $(y, z) = E_i$ where $G_i = (V_i, E_i)$. If $y, z \in V_{i-1}$, then $y \in Z$, as $Z$ is a downset. Otherwise $y = v_i$ or $z = v_i$. In the former case, we have $y = v_i \in a$, hence $y \in Z$, by hypothesis. In latter case ($z = v_i$), we have $y \in U_i \subseteq a$, hence $y \in Z$. In all cases, we have $y \in Z$, hence $Z$ is a closure in $G_i$.
  \end{description}

  We now consider the case where $v_i$ is removed from $X_i$, i.e., $X_i = X_{i-1} \setminus \set{v_i}$. In this case, $G_i = G_{i-1}$, so  $Z \subseteq V_i$ is a closed subset of $G_i$ if and only if it is a closed subset of $G_{i-1}$. Therefore, for any closed subset $Z$ in $G_i$ with $A = Z \cap X_{i}$, we have $Z \cap X_{i-1} = A$ or $A \cup \set{v_i}$ (and the two cases are clearly mutually exclusive). Therefore~(\ref{eqn:remove}) correctly computes $C_i(A)$.
\end{proof}

\begin{thm}
  \label{thm:downsets}
  Let $G$ be a directed acyclic graph with $n$ vertices and pathwidth $k$.  Given $G$ and a simple path decomposition $\calX$ of $G$ with width $k$, there is an algorithm that computes the number of closed subsets of $G$ in $O(2^k k n )$ time. 
  
%  $2^{O(\pw(H_\calP))} p$ time. 
%  There exists an algorithm $A$ that for any DAG $G = (V, E)$, $A$ computes the number of downsets in $G$ in time $2^{O(\pw(G))} n$. 
\end{thm}

\begin{proof} %[Proof of Theorem~\ref{thm:downsets}].
Our discussion above outlines the algorithm.  For $i \in [2n]$, $A \subseteq X_i$, compute $C_i(A)$ recursively using equations (\ref{eqn:insert}) and (\ref{eqn:remove}).  Return  $C_{2n}(\varnothing) + C_{2n}(X_{2n})$.   Lemma~\ref{lem:count-update} establishes the correctness of the computed values. 

%that all values $C_i(A)$ for all $i \in [2n]$, all $A \subseteq X_i$,  are computed correctly.  The total number of downsets of $G$ then is $C_{2n}(\varnothing) + C_{2n}(X_{2n})$. \\
%since every downset of $\calP$ either contains the only element in $X_{2p}$ or not. 

%[QUESTION:  Do we need to consider time to construct $H_\calP$ and the path decomposition $\calX$?] \\

  All that remains  is to prove the run-time. To this end, we note that each insertion and removal step requires updating the $2^{\abs{X_i}} \leq 2^{k+1}$ entries of $C_i$. Each computation of $C_i(A)$ can be done in $O(k)$ time by examining the neighborhood of $v_i$, and querying the required values of $C_{i-1}$. Finally, the algorithm terminates after $2n$ such updates, so the final run-time is $O(2^k kn)$.
 \end{proof}
 
 \begin{cor}
 Let $\calP=(P, \prec)$ be a poset with $p$ elements.  Let $G=(P,E)$ be a directed acyclic graph whose transitive reduction is the Hasse diagram $H_\calP$ of $\calP$.  Then the number of downsets of $\calP$ can be computed in time $O(2^{\pw(G)} p^c)$ time. 
 \end{cor}

\subsection{Sampling Downsets in Pathwidth Bounded DAGs}
\label{sec:sampling-downsets}

Here, we describe an FPT algorithm for sampling downsets uniformly at random in a DAG.

\begin{thm}
  \label{thm:sampling-downsets}
  There exists an algorithm $\SampleDownset$ that, for any DAG $G = (V, E)$, returns a downset $Z$ in $G$ sampled uniformly at random in time in time $2^{O(\pw(G))} n^{O(1)}$. 
\end{thm}

The idea of $\SampleDownset$ is simple. Let $G = (V, E)$ be a DAG, and $V = \set{v_1, v_2, \ldots, v_p}$ a topological sorting of $G$'s vertices. $A$ initially sets $Z = \varnothing$, and iterates through $v_1, v_2, \ldots$ choosing to add each $v_i$ in $Z$ with probability $p_i$. Specifically, $p_i$ is the proportion of downsets in $G$ that contain $v_i$ among all downsets whose intersection with $\set{v_1, v_2, \ldots, v_{i-1}}$ is $Z$. We call this procedure $\SampleDownset$ (Algorithm~\ref{alg:sample-downset}). We show that when the procedure terminates, each downset $Z$ is returned with probability $1 / \down(G)$, where $\down(G)$ denotes the number of downsets in $G$. In order to compute $p_i$, $\SampleDownset$ uses the algorithm of Theorem~\ref{thm:downsets} as a subroutine. We assume $\SampleDownset$ receives a (simple) path decomposition $\calX$ of $G$ as input. 

\begin{algorithm}
  \caption{$\SampleDownset(G, \calX)$}
  \label{alg:sample-downset}
  \begin{algorithmic}[1]
    \STATE $v_1, v_2, \ldots, v_p$ a topological sorting of vertices of $G$
    \STATE $Z \leftarrow \varnothing$
    \STATE $H \leftarrow G$
    \FOR{$i = 1$ \TO $n$}
    \IF{$v_i \in H$} \label{ln:check-condition}
    \STATE $a_i^{1} \leftarrow \down(H \setminus \set{v_i})$ \label{ln:ai1}
    \STATE $a_i^0 \leftarrow \down(H \setminus \desc(v_i))$ \label{ln:ai0}
    \STATE $r \leftarrow $ uniformly at random from $\set{1, 2, \ldots, a_i^1 + a_i^0}$
    \IF{$r \leq a_i^1$}\label{ln:include-condition}
    \STATE $Z \leftarrow Z \cup \set{v_i}$
    \STATE $H \leftarrow H \setminus \set{v_i}$
    \ELSE
    \STATE $H \leftarrow H \setminus \desc(v_i)$ \label{ln:not-added}
    \ENDIF\label{ln:include-condition-end}
    \ENDIF
    \ENDFOR
    \RETURN $Z$
  \end{algorithmic}
\end{algorithm}

[FIXME: Add intuition before proof]

\begin{proof}[Proof of Theorem~\ref{thm:sampling-downsets}]
  First we establish the correctness of $\SampleDownset$. Define the sequence of graphs $H_0 \supseteq H_1 \supseteq H_2 \supseteq \cdots \supseteq H_p$ where $H_0 = G$ and for $i \geq 1$, $H_i$ is the graph $H$ at the end of the $i\th$ iteration of the loop in $\SampleDownset$. Let $Z$ denote the (random) output of $\SampleDownset$, and let $z \in \set{0, 1}^p$ be the characteristic vector associated with $Z$ (i.e., $z_i = 1 \iff v_i \in Z$). Let $Y$ be any fixed subset of $G$, and let $y$ be $Y$'s characteristic vector. We will show that
  \begin{equation}
    \label{eqn:hitting-probability}
    \Pr(z = y) =
    \begin{cases}
      \frac{1}{\down(G)} &\text{if } Y \text{ is a downset in } G,\\
      0 &\text{otherwise.}
    \end{cases}
  \end{equation}
  Here, $\down(G)$ denotes the number of downsets in $G$.

  We first consider the case where $Y$ is not a downset. That is, there exist vertices $v_i$ and $v_j$ with $i < j$ such that there is a path from $v_i$ to $v_j$, and $v_i \notin Y$, $v_j \in Y$. Suppose that the output $Z$ of $\SampleDownset$ satisfies $z_i = y_i = 0$ (since $v_i \notin Y$). Since $v_i \notin Z$, during iteration $i$ of the loop in $\SampleDownset$, the algorithm must have executed Line~\ref{ln:not-added}, so that
  \[
  H_i = H_{i-1} \setminus \set{w \sucht \text{there is a directed path from } v_i \text{ to } w}.
  \]
  In particular, $v_j \notin H_i$. Therefore, $v_j \notin H_j$ (as $H_0 \supseteq H_1 \supseteq H_2 \cdots$), implying that $v_j$ was not added to $Z$ in iteration $j$ of the loop (due to the condition in Line~\ref{ln:check-condition}. Therefore, $z_i \neq y_i$, i.e., $\Pr(z = y) = 0$.

  Now consider the case where $Y$ is some fixed downset. Form the sequence of graphs $H_0' \supseteq H_1' \supseteq \cdots \supseteq H_p'$ where $H_0' = G$ and for $i \geq 1$,
  \[
  H_i' =
  \begin{cases}
    H_{i-1}' &\text{if } v_i \notin H_{i-1}'\\
    H_{i-1}' \setminus \set{v_i} &\text{if } v_i \in Y\\
    H_{i-1}' \setminus \desc(v_i) &\text{if } v_i \notin Y.
  \end{cases}
  \]
  Observe that for any $i \geq 1$, if $z_1 = y_1, z_2 = y_2, \ldots, z_{i-1} = y_{i-1}$, then we have $H_{i-1} = H_{i-1}'$. The condition in Line~\ref{ln:include-condition} is satisfied with probability
  \[
  p_i = \frac{\down(H_{i-1} \setminus \set{v_i})}{\down(H_{i-1} \setminus \set{v_i}) + \down(H_{i-1} \setminus \desc(v_i))}.
  \]
  Thus, if $y_i = 1$, then $H_i' = H_{i-1} \setminus \set{v_i}$, and conditioned on the event $z_1 = y_1, z_2 = y_2, \ldots, z_{i-1} = y_{i-1}$, the probability that $z_i = y_i$ is $p_i$. Similarly if $y_i = 0$, then $H_i' = H_{i-1} \setminus \desc(v_i)$, and (conditioned on the same event) the probability that $z_i = y_i$ is
  \[
  1 - p_i = \frac{\down(H_{i-1} \setminus \desc(v_i))}{\down(H_{i-1} \setminus \set{v_i}) + \down(H_{i-1} \setminus \desc(v_i)}.
  \]
  In either case, we obtain
  \begin{align*}
    \Pr\paren{z_i = y_i \sucht \forall j < i, z_j = y_j} &= \frac{\down(H_i')}{\down(H_{i-1} \setminus \set{v_i}) + \down(H_{i-1} \setminus \desc(v_i))}\\
    &= \frac{\down(H_i')}{\down(H_{i-1}' \setminus \set{v_i}) + \down(H_{i-1}' \setminus \desc(v_i))}\\
    &= \frac{\down(H_i')}{\down(H_{i-1}')}.
  \end{align*}
  The final equality holds because $\down(H_{i-1}' \setminus \set{v_i})$ counts the number of downsets in $H_{i-1}'$ that contain $v_i$, while $\down(H_{i-1}' \setminus \desc(v_i))$ counts the number of downsets that do not contain $v_i$. Hence, their sum is $\down(H_{i-1}')$. Finally, we apply the law of total probability to compute
  \begin{align*}
    \Pr(z = y) &= \Pr(\forall i,\, z_i = y_i)\\
    &= \prod_{i = 1}^p \Pr\paren{z_i = y_i \sucht \forall j < i,\, z_j = y_j}\\
    &= \prod_{i = 1}^p \frac{\down(H_i')}{\down(H_{i-1}')}\\
    &= \frac{\down(H_p')}{\down(H_0')}\\
    &= \frac{1}{\down(G)}.
  \end{align*}
  The final equality holds because $H_p' = \varnothing$ (hence $\down(H_p') = 1$), and $H_0' = G$. This gives the correctness of $\SampleDownset$.

  As for the algorithm's runtime, suppose $k = \pw(G)$, the pathwidth of the original graph. Since each graph $H_i$ is a subgraph of $G$, we have $\pw(H_i) \leq k$ for all $k$. Therefore, by Theorem~\ref{thm:downsets} the computations of $a_i^1$ and $a_i^0$ in Lines~\ref{ln:ai1} and~\ref{ln:ai0} can be performed in time $2^{O(k)} \cdot O(p)$. All other operations can be performed in time $O(k \cdot p)$ per iteration of the main loop. Since the algorithm terminates after $p$ iterations, the overall runtime of the algorithm is $2^{O(k)} O(k \cdot p^2) = 2^{O(k)} O(p^2)$, as desired.
\end{proof}

